Integration Methods and Accelerated Optimization Algorithms

We show that accelerated optimization methods can be seen as particular instances of multi-step integration schemes from numerical analysis, applied to the gradient flow equation. In comparison with recent advances in this vein, the differential equation considered here is the basic gradient flow and we show that multi-step schemes allow integration of this differential equation using larger step sizes, thus intuitively explaining acceleration results.

==> sections/abstract.tex <==

\begin{abstract}
	Stuff
	%In this paper we recall the important properties of a particular Ordinary Dfferential Equation (ODE), the Gradient flow, under the hypothesis of smoothness and strong convexity. Then we will summarize the main results in the theory of integration methods, like stability and convergence. Then we show strong links between optimization algorithms and these integration methods applied gradient flow.
\end{abstract}

\begin{keywords}
	List of keywords
\end{keywords} 


==> sections/interpretation.tex <==
\begin{proposition-non}
	A method is consistent if and only if
	\BEAS
	\rho(1) = 0 \qquad \text{and} \qquad \rho'(1) = \sigma(1).
	\EEAS
\end{proposition-non}

\paragraph{First condition, $\rho(1) = 0$.} If the condition is not satisfied, then the method exhibits an artificial gain or damping. Assume we start at some equilibrium $x^*$ of \ref{eq:ode} (i.e. $\nabla f(x^*) =0$), so $x_{i}=x^*$ for the first $s-1$ steps. The next iterate becomes
\[
x_s = -\sum_{i=0}^{s-1} \rho_{i} x^* + h \sigma(E) \underbrace{ g(x^*) }_{ =0 },
\]
and if $1+\sum_{i=0}^{s} \rho_{i} = \rho(1)\neq 0$, we have that the next iterate $x_s$ is different from $x^*$.

\paragraph{Second condition, $\rho'(1) = \sigma(1)$.} If this relation is not satisfied, we actually are integrating another equation than \eqref{eq:ode}. Assuming the first condition satisfied is a root of $\rho$, consider the factorization
\[
\rho(z) = (z-1) \tilde \rho(z) \qquad \Rightarrow \qquad \tilde \rho(1) = \rho'(1) ,
\]
where $\tilde \rho$ is a polynomial of degree $s-1$, and $\rho'(1) = \tilde \rho (1)$. The linear multi-step method becomes
\[
\tilde\rho(E) (y_{k+1}-y_k)  = h\sigma(E) g(y_0).
\]
Let $G_k = \sum_{i=1}^k hg(x_i)$. If we sum up the above equation from $k=0$, the relation becomes
\[
	\tilde\rho(E) (y_{k}-y_0)  = \sigma(E) G_k.
\]
If $h$ goes to zero, our iterates $x_k$ converge to some continuous curve $c(t)$, and $G_k \rightarrow \int_{0}^{t} g(c(\tau)) \dif \tau$,
\[
	\tilde{\rho}(E)(c(t)-x(0)) = \tilde{\rho}(1)(c(t)-x(0)) = \sigma(1)\int_{t_0}^{t} g(c(\tau)) \dif \tau,
\]
using $Ec(t) = c(t)$. If we take the derivative over time,
\BEAS
\tilde\rho(1)\dot c(t) & = & \sigma(1) g(c(t))\\
\Leftrightarrow \quad \rho'(1) \dot c(t) & = & \sigma(1) g(c(t)).
\EEAS
Since we would like to have $c(t) = x(t)$, the solution of \eqref{eq:ode}, we absolutely need $\rho'(1)$ = $\sigma(1)$.

